Evaluating Beam Sweeping for AoA Estimation with an RIS Prototype: Indoor/Outdoor Field Trials

Reconfigurable Intelligent Surfaces (RISs) have emerged as a promising technology to enhance wireless communication systems by enabling dynamic control over the propagation environment. However, practical experiments are crucial towards the validation of the theoretical potential of RISs while establishing their real-world applicability, especially since most studies rely on simplified models and lack comprehensive field trials. In this paper, we present an efficient method for configuring a $1$-bit RIS prototype at sub-$6$ GHz, resulting in a codebook oriented for beam sweeping; an essential protocol for initial access and Angle of Arrival (AoA) estimation. The measured radiation patterns of the RIS validate the theoretical model, demonstrating consistency between the experimental results and the predicted beamforming behavior. Furthermore, we experimentally prove that RIS can alter channel properties and by harnessing the diversity it provides, we evaluate beam sweeping as an AoA estimation technique. Finally, we investigate the frequency selectivity of the RIS and propose an approach to address indoor challenges by leveraging the geometry of environment.

==> mycompress.tex <==
\setlength{\textfloatsep}{1pt plus 0pt minus 2.0pt}		% space between last top float or first bottom float and the text
\setlength{\floatsep}{0pt plus 0pt minus 2.0pt}			% space left between floats
\setlength{\dblfloatsep}{0pt plus 0pt minus 2.0pt}			% space left between floats
\setlength{\dbltextfloatsep}{0pt plus 0pt minus 2.0pt}			% space left between floats
\setlength{\abovecaptionskip}{0pt plus 0pt minus 10pt}	% space above caption
\setlength{\belowcaptionskip}{0pt plus 0pt minus 3pt}	% space below caption
\setlength{\abovedisplayskip}{2pt plus 1pt minus 2pt}	% space before maths
\setlength{\belowdisplayskip}{2pt plus 1pt minus 2pt}	% space after maths

\renewcommand{\topfraction}{0.90}
\renewcommand{\bottomfraction}{0.90}
\renewcommand{\floatpagefraction}{0.9}
\renewcommand{\textfraction}{0.02}
%extra compression with title spacings

\usepackage{titlesec}
\titlespacing*{\section}{0pt}{0pt plus 0pt minus 0pt}{0pt plus 1pt minus 5pt}
\titlespacing{\subsection}{0pt}{1pt plus 0pt minus 1pt}{0pt plus 0pt minus 1pt}
\titlespacing{\subsubsection}{0pt}{1pt plus 0pt minus 12pt}{1pt}

